Asynchronous Bounded Expected Delay Networks

The commonly used asynchronous bounded delay (ABD) network models assume a fixed bound on message delay. We propose a probabilistic network model, called asynchronous bounded expected delay (ABE) model. Instead of a strict bound, the ABE model requires only a bound on the expected message delay. While the conditions of ABD networks restrict the set of possible executions, in ABE networks all asynchronous executions are possible, but executions with extremely long delays are less probable. In contrast to ABD networks, ABE networks cannot be synchronised efficiently. At the example of an election algorithm, we show that the minimal assumptions of ABE networks are sufficient for the development of efficient algorithms. For anonymous, unidirectional ABE rings of known size N we devise a probabilistic leader election algorithm having average message and time complexity O(N).

==> related.tex <==
There exists a broad range of leader election algorithms; among them also for anonymous networks. We compare our algorithm with the algorithms that have similar ideas as well as the ones that have linear time or message complexity.

% Itai and Rodeh \cite{IR81,IR90} studied how to break the symmetry in anonymous networks using probabilistic algorithms. In \cite{IR81}, a leader election algorithm for asynchronous anonymous unidirectional rings with a known size is presented. The algorithm terminates with probability one\footnote{It exhibits infinite traces, but the probability that such an infinite trace is executed is zero}; its has average message complexity $\complex{\netsize\log \netsize}$ and on average transmits $\complex{\netsize \log^2 \netsize}$ bits. It proceeds in election rounds. A message carries hop counter to recognise its source. Moreover, it is equipped with the additional data: random identifier (ID), current election round number to enforce FIFO message order and a boolean to detect a name clash. Active processes with the largest ID deactivate other nodes, until there is only one active node left.

Without restoring to probabilistic solutions,
several papers~\cite{BP89,Hua93,ILS95,FJ01}
present leader election algorithms for anonymous rings of prime size.
More recently, with the population protocol model~\cite{AR07},
Angluin et al.~\cite{AAFJ05} construct a self-stabilising leader election algorithm for anonymous,
asynchronous rings of odd size. 
Fischer and Jiang~\cite{FJ06} give a self-stabilising leader election algorithm for
anonymous, asynchronous rings, augmented with an oracle $\Omega$? for leader detection.
The detector may give wrong answers sometimes,
but it will eventually return a correct answer permanently.

% \todo{Cite \cite{129767} and compare their approach with our ABE networks}
